Extending the Range of Drone-based Delivery Services by Exploration

Drones have a fairly short range due to their limited battery life. We propose an adaptive exploration techniques to extend the range of drones by taking advantage of physical structures such as tall buildings and trees in urban environments. Our goal is to extend the coverage of a drone delivery service by generating paths for a drone to reach its destination while learning about the energy consumption on each edge on its path in order to optimize its range for future missions. We evaluated the performance of our exploration strategy in finding the set of all reachable destinations in a city, and found that exploring locations near the boundary of the reachable sets according to the current energy model can speed up the learning process.

==> 5-prs.tex <==
\section{Probabilistic Reachable Sets}
\label{sec:pmodel}

In this section, we consider the case in which $u(e; l, s, d)$ follows a normal
distribution $N(\mu_{e}, \sigma_{e}^2)$, where $\mu_{e}$ and $\sigma_{e}^2$ are
the mean and variance of $u(e; l, s, d)$, respectively.  Although the
assumption of normality is not always correct, it is an appropriate assumption
without further knowledge about the distribution.

Let $M^t_{l,s,d} = \{ (\mu_{e}, \sigma_{e}^2) : e \in \Eunknown_{l, s, d} \}$ be
an energy model under $(l,s,d)$ at time $t$.  We define a notion of reachable sets whose
destinations are \emph{probabilistically} reachable based on energy models as
follows.  Given a certain amount of $\Energy'$, a drone can successfully
traverse $\rho$ if 
\begin{equation}
\small
  \sum_{e \in \known(\rho)} \energy(e; l, s, d) + \sum_{e \in \unknown(\rho)} u(e; l, s, d) \leq \Energy'.
  \label{eq:pathconstraint}
\end{equation}
Let $P(\rho; \Energy', l, s, d)$ be the \emph{probability of success}
of traversing a path $\rho$ using a maximum amount of energy $\Energy'$:
\begin{equation}
  P(\rho; \Energy', l, s, d) = P(X' \leq C') = P(Z \leq \frac{C' - \mu_\rho}{\sigma_\rho}),
  \label{eq:path_prob}
\end{equation}
where $X' = \sum_{e \in \unknown(\rho)} u(e; l, s, d)$ and $C' = \Energy' - \sum_{e \in \known(\rho)} \energy(e; l, s, d)$. Basically, $P(\rho; \Energy', l, s, d)$ is the probability that
Inequality~\ref{eq:pathconstraint} is true.


% $P(\rho; \Energy', l, s, d)$ can be calculated as follows.  
% Let   Since the sum of normal distributions is also a normal
% distribution, $X'$ follows a normal distribution $N(\mu_\rho, \sigma_\rho^2)$,
% where $\mu_\rho = \sum_{e \in \unknown(\rho)}{\mu_e}$, $\sigma_\rho^2 = \sum_{e
% \in \unknown(\rho)}{\sigma_e^2}$, where $\mu_e$ and $\sigma_e^2$ are given
% in $M_{l,s,d}$.  $P(\rho; \Energy', l, s, d)$ is the probability that
% Inequality~\ref{eq:pathconstraint} is true. Hence,
% \begin{equation}
%   P(\rho; \Energy', l, s, d) = P(X' \leq C') = P(Z \leq \frac{C' - \mu_\rho}{\sigma_\rho}),
%   \label{eq:path_prob}
% \end{equation}
% which can be calculated by using the probability table of the standard normal
% distribution of $Z$ that is available in many software libraries.




% Based on the definition of the probability of success of a path,

Then we define the probability of success of a trip as follows.
Let $\tau = \rho_1 \oplus \rho_2$, where 
$\rho_1$ is a path connecting $v_0$ to $\vdest$ and
$\rho_2$ is a path connecting $\vdest$ to $v_0$.
Given a certain amount of $\Energy$, a drone can successfully traverse $\tau$ if
{\small
\begin{multline}
  \sum_{e \in \known(\rho_1)} \energy(e; l, s, d) + \sum_{e \in \unknown(\rho_1)} u(e; l, s, d) + \\
  \sum_{e \in \known(\rho_2)} \energy(e; 0, s, d) + \sum_{e \in \unknown(\rho_2)} u(e; 0, s, d) \leq \Energy.
  \label{eq:tripconstraint}
\end{multline}
}

The probability of success of $\tau$, i.e., the probability that the
Inequality~\ref{eq:tripconstraint} is true, is
\begin{equation}
  P(\tau; \Energy, l, s, d) = P(X \leq C) = P(Z \leq \frac{C - \mu_\tau}{\sigma_\tau}),
  \label{eq:trip_prob}
\end{equation}
where $X = \sum_{e \in \unknown(\rho_1)} u(e; l, s, d) + \sum_{e \in
\unknown(\rho_2)} u(e; 0, s, d)$, $C = \Energy - \sum_{e \in \known(\rho_1)}
\energy(e; l, s, d) - \sum_{e \in \known(\rho_2)} \energy(e; 0, s, d)$,
% $X$ follows a normal distribution $N(\mu_\tau, \sigma_\tau^2)$,
% where 
$ \mu_\tau = \sum_{e \in \unknown(\rho_1)}{\mu_e} + \sum_{e' \in \unknown(\rho_2)}{\mu_{e'}}$,
and
$\sigma_\tau^2 = \sum_{e \in \unknown(\rho_1)}{\sigma_e^2} + \sum_{e' \in \unknown(\rho_2)}{\sigma_{e'}^2}$,
in which $\mu_e$ and $\sigma_e^2$ are given by $M_{l,s,d}$ 
and $\mu_{e'}$ and $\sigma_{e'}^2$ are given by $M_{0,s,d}$.

Given energy models $M^t_{l,s,d}$ and $M^t_{0,s,d}$, the maximum probability of
reaching a destination $\vdest$ is
\begin{equation}
P_{\max}(\vdest) = \max_{\tau} P(\tau; \Energy, l, s, d),
\end{equation}
where $\tau$ is any trip to $\vdest$.  We define $D^t_{l,s,d,\phi} = \{ \vdest :
\vdest \in D \text{ and } P_{\max}(\vdest) \geq \phi \}$ to be the
\emph{probabilistic reachable set} under $(l,s,d)$ and $\phi$.  It means that
according to the energy models $M^t_{l,s,d}$ and $M^t_{0,s,d}$, for each
destination $\vdest \in D^t_{l,s,d,\phi}$ there is a trip $\tau$ to $\vdest$ such
that $P(\tau; \Energy, l, s, d) \geq \phi$.

% Computing $P_{\max}(\vdest)$ can be difficult since it involves an enumeration
% of all possible trips.  Therefore sampling methods can be used to estimate
% $D_{l,s,d,\phi}$: for each destination $v$ if we find a trip $\tau$,
% among some randomly generated trips to $v$, such that $P(\tau; \Energy, l, s, d) \geq
% \phi$, we know that $v \in D_{l,s,d,\phi}$.  
% While this method will yield a subset of $D_{l,s,d,\phi}$ only,
% the subset will approach $D_{l,s,d,\phi}$ as the number of sampling increases.

{\bf Model Update:}
Equation~\ref{eq:regression} provides a way to distribute
the measurement of an unknown to other unknowns in an energy model.
Given an energy model $M^{t}_{l,s,d}$ at time $t$ 
and a measurement of the unknown on edge $e'$,
we compute the energy model $M^{t+1}_{l,s,d} = \{ \{ (\mu_{e,t+1},
\sigma_{e,t+1}^2) : e \in \Eunknown_{l, s, d} \setminus \{ e' \} \} $ at time
$t+1$ using these equations:
\begin{align}
\mu_{e,t+1} & = \frac{w_t \mu_{e,t} + w_{e} \hat{\energy}(e; l, s, d) }{w_t + w_{e}} \\
\eta_{e,t+1}^2 & = \frac{w_t \eta_{e,t}^2 + w_{e} \hat{\energy}(e; l, s, d)^2 }{w_t + w_{e}} \\
\sigma_{e,t+1}^2 &= \eta_{e,t+1}^2 - \mu_{e,t+1}^2\\
w_{t+1} &= w_t + w_{e},
\end{align}
where $w_t$ is the accumulative weight including the prior,  for all $e \in \Eunknown_{l, s, d} \setminus \{ e' \}$.



% Given a configuration $(l, s, d)$, we partition the set of edges $E$ into two
% sets: $\Eknown_{l, s, d}$ and $\Eunknown_{l, s, d}$, where $\Eunknown_{l, s,
% d}$ is the set of all edges whose energy consumption are currently unknowns.
% For each $e \in \Eunknown_{l, s, d}$, let $u(e; l, s, d)$ be a random variable
% for $\energy(e; l, s, d)$.  

% First, we partition the set of edges on a path $\rho$ into
% two sets:
% $\known(\rho) = \{ e \in \rho : e \in \Eknown_{l, s, d} \}$ and 
% $\unknown(\rho) = \{ e \in \rho : e \in \Eunknown_{l, s, d} \}$.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 6-safe.tex <==
\section{$\kappa$-Safe Trips}
\label{sec:safe}

% To begin with, we model the energy consumption on an edge $e_i$ associated with
% a set of parameter $l,s,d$ as a Normal distribution: $u(e_i;l,s,d) =
% N(\mu_\rho, \sigma_\rho^2)$ of which mean and variance would be updated after
% each time the drone operates and collects information about the map. Given a
% trip $\tau$, if we call $X$ the total energy consumption on this trip, we have
% $X = \sum_{e \in \tau} \energy(e; l, s, d)$. It is clear that $X$ follows a
% Normal distribution. Therefore, if we call $P(\tau; \Energy, l, s, d)$ as the
% probability of success of the trip $\tau$, we can easily compute this value
% based on Equation~\ref{eq:trip_prob}. 
% \begin{equation}
%   P(\tau; \Energy, l, s, d) = P(X \leq \Energy)
%   \label{eq:trip_prob}
% \end{equation}

% As the drone gather more and more information about energy consumption, this
% computation is more and more accurate thanks to an updating process. The
% updating process consists of two steps: 1) update mean and variance of the same
% explored edges but with other sets of $l,s,d$. This can be accomplished using
% linear regression method; 2) update mean and variance of neighbor edges with
% different sets of $l,s,d$. \commentt{This step is performed by using Gaussian
% process regression.  \commentt{Due to the lack of space, we omit here}.}


% Let $\Eunknown_{l, s, d} \subseteq E$ be the set of all edges whose
% energy consumption are unknowns under a configuration $(l,s,d)$.  Let
% $U_{l,s,d}$ be a set of all random variables about the energy consumption of
% the edges in $G$ If $u_1 \in U_{l, s, d}$ is a random variable representing
% the unknown energy consumption of $e_i \in \Eunknown_{l, s, d}$. 
% Let $\Eknown_{l, s, d} = E \setminus \Eunknown_{l, s, d}$ be the set of all
% edges whose energy consumption is known. 

% For instance, this failure occurs when there is an edge with unknown energy
% consumption that requires a lot of energy to traverse, but the drone finds out
% it run out of energy only after it traverses the edge.  Since there is always a
% small chance that a drone will fail in a trip and drones are expensive, 

% As long as a trip $\tau$ involves some edges with unknown energy consumption,
% the probability of success of $\tau$ is less than $1$, meaning that there is a
% non-zero chance that the drone will fail to deliver the package or fail to
% return to the base after delivering the package.  Until now we ignored this
% issue and assumed that when a drone fails to return to the distribution center, it
% will land safely and some one will pick it up later.  However, 

It would be ideal if we can ensure that a drone returns to the base with a
high probability even if it fails to deliver the package.  Hence, we
define a contingency plan that has a minimum probability of $\kappa$ of
returning to the base if it discovers that it is unlikely to
deliver the package. We call such contingency plan a \emph{$\kappa$-safe trip}.
In essence, a $\kappa$-safe trip is a trip augmented with \emph{backup paths} at
each node that the drone can use if it has to return to the base
immediately.  
% Algorithm~\ref{alg:controller} is the pseudo-code of the drone's controller that utilizes backup plans.
The drone takes a trip $\tau$ whose probability of success $P(\tau; \Energy, l, s, d)$,
as computed in Equation~\ref{eq:trip_prob}, is at least $\phi$.
The controller will then instruct the drone to traverse the graph according to $\tau$.
During the traversal, the controller will check whether the probability
$P(\tau'; \Energy', l, s, d)$ of the remaining path $\tau'$ on $\tau$ to $\vdest$ is
at least $\phi$. This probability can be computed by
\begin{equation}
  P(\tau'; \Energy', l, s, d) = P(X \leq C) = P(Z \leq \frac{C - \mu_{\tau'}}{\sigma_{\tau'}}),
  \label{eq:remain_prob}
\end{equation}
where
\begin{small_ind_s_itemize}
\item $\rho_1 = \langle e_1, e_2, \ldots, e_k \rangle$ and
      $\rho_2 = \langle e_{k+1}, e_{k+2}, \ldots, e_n \rangle$,
      where $\rho_1$ and $\rho_2$ are the paths on $\tau'$ before and
      after $\vdest$, respectively.
\item $X = \sum_{e \in \unknown(\rho_1)} u(e; l, s, d) + \sum_{e \in \unknown(\rho_2)} u(e; 0, s, d)$;
\item $C = \Energy' - \sum_{e \in \known(\rho_1)} \energy(e; l, s, d) - \sum_{e \in \known(\rho_2)} \energy(e; 0, s, d)$.
\item $\mu_{\tau'} = \sum_{e \in \unknown(\rho_1)}{\mu_e} + \sum_{e' \in \unknown(\rho_2)}{\mu_{e'}}$; and
\item $\sigma_{\tau'}^2 = \sum_{e \in \unknown(\rho_1)}{\sigma_e^2} + \sum_{e' \in \unknown(\rho_2)}{\sigma_{e'}^2}$.
\end{small_ind_s_itemize}


% \begin{algorithm}[t]
% \caption{A drone controller that utilizes backup paths}
% \label{alg:controller}
% \begin{algorithmic}[1]
% \footnotesize
% \Procedure{Deliver}{$\tau$, \textsf{Backup}, $\Energy$ $v_0$, $\vdest$, $l$, $s$, $d$, $\kappa$ }
%   \State Let $\tau' = \tau$ be the remaining edges on $\tau$
%   \State Let $\Energy' = \Energy$ be the remaining energy
%   \State Let $v = v_0$ be the current node
%   \State ${\sf isFail} \assign \False$
%   \While {${\sf isFail} = \False$ and $v \neq \vdest$}
%     \If { $P(\tau'; \Energy', l, s, d) \geq \phi$ }
%       \State Let $e$ be the first edge in $\tau'$
%       \State remove $e$ from $\tau'$
%       \State Traverse $e$ and measure $\energy' = \energy(e; l, s, d)$
%       \If {$e \in \Eunknown_{l, s, d}$}
%         \State $u' \assign \energy'$ where $u' = u(e; l, s, d)$
%         \State $E' \assign \{ e' \in \Eunknown_{l, s, d} : u(e'; l, s, d) = u' \}$
%         \State $\Eunknown_{l, s, d} \assign \Eunknown_{l, s, d} \setminus E'$
%         \State $\Eknown_{l, s, d} \assign \Eknown_{l, s, d} \cup E'$
%       \EndIf
%       \State $\Energy' \assign \Energy' - \energy'$; $v \assign \vend$ where $e = (v, \vend)$.
%     \Else
%       \State ${\sf isFail} = \True$
%     \EndIf
%   \EndWhile
%   \If {$v = \vdest$}  \hspace{.1in} \textsf{// The drone has reached $\vdest$}
%     \State \textsc{GoToCenter}($\tau'$, $\Energy'$, $v$, $v_0$, $0$, $s$, $d$)
%   \Else  \hspace{.1in} \textsf{// The drone did not reach $\vdest$}
%     \State \textsc{GoToCenter}($\textsf{Backup}(v)$, $\Energy'$, $v$, $v_0$, $l$, $s$, $d$)
%   \EndIf
% \EndProcedure
% \Procedure{GoToCenter}{$\rho$, $\Energy'$, $v$, $v_0$, $l$, $s$, $d$}
%   \State Let $\rho' = \rho$ be the remaining edges on $\rho$
%   \While {$v \neq v_0$}
%     \State Let $e$ be the first edge in $\rho'$; remove $e$ from $\rho'$
%     \State Traverse $e$ and measure $\energy' = \energy(e; l, s, d)$
%     \If {$e \in \Eunknown_{l, s, d}$}
%       \State $u' \assign \energy'$ where $u' = u(e; l, s, d)$
%       \State $E' \assign \{ e' \in \Eunknown_{l, s, d} : u(e'; l, s, d) = u' \}$
%       \State $\Eunknown_{l, s, d} \assign \Eunknown_{l, s, d} \setminus E'$
%       \State $\Eknown_{l, s, d} \assign \Eknown_{l, s, d} \cup E'$
%     \EndIf
%     \State $\Energy' \assign \Energy' - \energy'$; $v \assign \vend$ where $e = (v, \vend)$.
%   \EndWhile
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

\noindent
If $P(\tau'; \Energy', l, s, d)$ is less than $\phi$ at any node on its path to
$\vdest$, we deem that it is unsafe for the drone to continue and it
should return to the base immediately.  We have to pre-compute a
set of backup paths for all nodes towards $\vdest$ on $\tau$
such that a drone can follow the backup path to go back to the base if needed.
Let $\Backup$ be a mapping from the set of nodes on $\tau$ to a set of backup paths.
Suppose we are given a backup path $\rho = \Backup(v)$ at $v$.
We require that the probability of success of $\rho$ must be at least
$\kappa$.  However, the probability of
success of $\rho$ \emph{cannot} be computed by Equation~\ref{eq:trip_prob},
because when a drone has to return to the base, it already knows
that $P(\tau'; \Energy', l, s, d)$ is less than $\phi$.  Hence, the probability
of success of $\rho$ must be a conditional probability that depends on the
condition $P(\tau'; \Energy', l, s, d) < \phi$.

When $P(\tau'; \Energy', l, s, d) < \phi$ at node $v$, it means that the energy
consumed on the path from $v_0$ to $v$ is too much, causing difficulty in
finishing the trip.  From Equation~\ref{eq:remain_prob}, we can compute the
minimum $\Energy'$ that causes $P(\tau'; \Energy', l, s, d) < \phi$: $P(\tau';
\Energy', l, s, d) = P(X \leq C) = P(Z \leq \frac{C -
\mu_{\tau'}}{\sigma_{\tau'}}) < \phi$ if and only if
\begin{equation}
  \frac{C - \mu_{\tau'}}{\sigma_{\tau'}} < Q
  \label{eq:minE}
\end{equation}
where 
$\mu_{\tau'} = \sum_{e \in \unknown(\rho_1)}{\mu_e} + \sum_{e' \in \unknown(\rho_2)}{\mu_{e'}}$ and
$\sigma_{\tau'} = \sqrt{\sum_{e \in \unknown(\rho_1)}{\sigma_e^2} + \sum_{e' \in \unknown(\rho_2)}{\sigma_{e'}^2}}$. Furthermore, we can find the value of $Q$ such that $P(Z \leq Q) = \phi$ from the standard normal distribution table.  Then from Inequality~\ref{eq:minE}, we get $\Energy' < \Energy''$, where
\begin{multline*}
\Energy'' = Q \sigma_{\tau'} + \mu_{\tau'} + \\
\sum_{e \in \known(\rho_1)} \energy(e; l, s, d) + \sum_{e \in \known(\rho_2)} \energy(e; 0, s, d).
\end{multline*}
Hence, if $P(\tau';\Energy', l, s, d) < \phi$ at $v$, 
the minimum energy that has been consumed between $v_0$ and $v$
must be more than $\Delta(v) = \Energy - \Energy''$. In fact,
we can compute $\Delta(v)$ exactly for all $v$ on $\tau$ between $v_0$ and $\vdest$
before the drone leaves the base.

Given a node $v$ on $\tau$ between $v_0$ and $\vdest$,
let $\rho$ be the path on $\tau$ between $v_0$ and $v$.
Then the total energy consumption on $\rho$ is a 
\emph{truncated} normal distribution $X \sim N(\mu, \sigma^2)$ in the interval
$X > \Delta(v)$, where 
$\mu = \sum_{e \in \known(\rho)} \energy(e;l, s, d) + \sum_{e \in \unknown(\rho)}{\mu_e}$ and
 $\sigma^2 = \sum_{e \in \unknown(\rho)}{\sigma_e^2}$.
Let $\rho' = \Backup(v)$ be a backup path from $v$ to $v_0$.
Then the total energy consumption on $\rho'$ is a normal distribution 
$Y \sim N(\mu', \sigma'^2)$,
where $\mu' = \sum_{e \in \known(\rho')} \energy(e;l, s, d) + \sum_{e \in \unknown(\rho')}{\mu_e}$ and $\sigma'^2 = \sum_{e \in \unknown(\rho')}{\sigma_e^2}$.
Since the total energy consumption on $\rho$ and $\rho'$ is $X+Y$,
we define the probability of success of $\rho'$ to be
$P_{\sf truncated}(\rho'; \Energy, l, s, d) = P(X + Y \leq \Energy)$.

Based on this definition of the probability of success of a backup path, we define 
a \emph{$\kappa$-safe trip} to be a contingency plan with
two components: $(\tau, \Backup)$, which satisfies the following two conditions:
(1) $P(\tau; \Energy, l, s, d) \geq \kappa$; and
(2) For any node $v$ on $\tau$ before reaching $\vdest$,
$\Backup(v)$ is a path from $v$ to $v_0$ such
that $P_{\sf truncated}(\Backup(v); \Energy, l, s, d) \geq \kappa$.
A drone with a $\kappa$-safe trip $(\tau, \Backup)$
will have a probability of success of at least $\kappa$ to
return to the base whenever it discovers that the chance to successfully
deliver the package and return to the base is smaller than $\phi$.

One last issue with this approach is that when a drone flies on an unexplored edge, the edge can be too long and the drone can take too much energy to explore this particular edge and fail to return to the previous node and then follow the backup path of the previous node. To resolve this issue, the drone should set aside a fixed amount of \emph{reserved energy} for it to return the previous node, and this reserved energy is not used for calculating the $\kappa$-safe trips and is excluded from $\Energy$ in Algorithm~1. Since we do not model the energy consumption between any two points on an edge, we cannot calculate exactly how much reserved energy is needed.  However, if we assume the maximum energy for flying any edge in a map in the worst condition is $e_{\sf max}$, we can set the reserved energy to be equal to $2 e_{\sf max}$, such that when a drone has used more than $e_{\sf max}$ energy to explore an edge, it should immediately turn around and use the remaining half of the reserved energy to return to the previous node.

The notion of $\kappa$-safe trips is based on the assumption that the unknown energy consumption of an edge follows normal distributions whose long tail of probability means that a drone could possibly use a excessive large amount energy to fly on an edge.  Since $\kappa$ cannot be set to $1$ since no return path $\Backup(v)$ that involves some unknowns has $P_{\sf truncated}(\Backup(v); \Energy, l, s, d) = 1$, there is always a non-zero probability of losing a drone.  We could have avoided this issue by assuming we know the maximum amount of energy a drone take to fly on each edge. Then the backup paths can be computed by finding the shortest paths in a graph whose weights
are the maximum amount of energy of flying the edges.  These shortest paths will guarantee
to return to the base according to the new assumption. However, this approach is quite conservative and does not make use of the knowledge the drone learns in previous flight.  In practice, if we set $\kappa$ is high enough, the drone is quite safe.  In our experiments, we set $\kappa$ to $0.95$ and the number of lost drones is almost zero.



% \[
% P(\tau; l, s, d) =
% \left\{
%   \begin{array}{ll}
%     P(p_1; l, s, d) \times P(p_1; l, s, d) & mbox{if} \\
%     P(p; l, s, d) & \mbox{otherwise} \\
%   \end{array}
% \right.
% \]



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> Makefile <==
CONTENTDIR = .
MasterFilename = main

latexExe = pdflatex
latexOption =
SourceFiles = $(MasterFilename).tex $(CONTENTDIR)/*.tex $(CONTENTDIR)/bib/*.bib
Viewer = open -a Skim.app 

OriginalRefBib = $(HOME)/Documents/Bibdesk\ Database/bib/ref.bib
OriginalRefBibSrc = $(HOME)/Documents/Bibdesk\ Database/bib/bibdesk.bib
OriginalRefBibClean = $(HOME)/Documents/Bibdesk\ Database/bib/clean.pl


all:
	$(latexExe) $(latexOption) $(MasterFilename)

full: $(SourceFiles)
	@echo ----------------------------------------------------------------
	@echo --- Step 1 -----------------------------------------------------
	@echo ----------------------------------------------------------------
	$(latexExe) $(latexOption) $(MasterFilename)
	@echo ----------------------------------------------------------------
	@echo --- Step 2 -----------------------------------------------------
	@echo ----------------------------------------------------------------
	bibtex $(MasterFilename)
	@echo ----------------------------------------------------------------
	@echo --- Step 3 -----------------------------------------------------
	@echo ----------------------------------------------------------------
	$(latexExe) $(latexOption) $(MasterFilename)
	@echo ----------------------------------------------------------------
	@echo --- Step 4 -----------------------------------------------------
	@echo ----------------------------------------------------------------
	$(latexExe) $(latexOption) $(MasterFilename)

ref: $(OriginalRefBib)
	$(OriginalRefBibClean)
	cp -f $(OriginalRefBib) bib/auto.bib

view: $(MasterFilename).pdf
	$(Viewer) $(MasterFilename).pdf &


diff:
#	latexdiff --flatten ../2015-IWPSS-v4/main.tex main.tex > diff.tex
#	$(latexExe) diff.tex

clean:
	rm -f *.idx *.ilg *.ind *.out *.toc *.aux *.log *.bbl *.blg *lof *.lot *.dvi *.ps *.pdf missfont.log texput.log *.pdfsync *.rel *~
	rm -rf auto


